Equilibria of Dynamic Games with Many Players: Existence, Approximation, and Market Structure

In this paper we study stochastic dynamic games with many players; these are a fundamental model for a wide range of economic applications. The standard solution concept for such games is Markov perfect equilibrium (MPE), but it is well known that MPE computation becomes intractable as the number of players increases. We instead consider the notion of stationary equilibrium (SE), where players optimize assuming the empirical distribution of others' states remains constant at its long run average. We make two main contributions. First, we provide a rigorous justification for using SE. In particular, we provide a parsimonious collection of exogenous conditions over model primitives that guarantee existence of SE, and ensure that an appropriate approximation property to MPE holds, in a general model with possibly unbounded state spaces. Second, we draw a significant connection between the validity of SE, and market structure: under the same conditions that imply SE exist and approximates MPE well, the market becomes fragmented in the limit of many firms. To illustrate this connection, we study in detail a series of dynamic oligopoly examples. These examples show that our conditions enforce a form of "decreasing returns to larger states"; this yields fragmented industries in the limit. By contrast, violation of these conditions suggests "increasing returns to larger states" and potential market concentration. In that sense, our work uses a fully dynamic framework to also contribute to a longstanding issue in industrial organization: understanding the determinants of market structure in different industries.

==> extensions.tex <==
\delrj{
\section{Extensions}
\label{sec:extensions}

In this section we consider two extensions to the basic model
  presented thus far.  First, we consider a model where players may be
  {\em heterogeneous}; that is, they may not share the same payoff
  function or transition kernel.  Second, we consider a model where
  players may be coupled through their current {\em actions} as well
  as their states.

\subsection{Heterogeneous Players}

In this section, we study anonymous stochastic games with ex-ante heterogeneous
players. To represent this heterogeneity, at the beginning of the
game, a player is assigned a {\em type} (denoted by $\theta$)
that stays fixed for the entire duration of the game. For simplicity,
we assume that the players'
types are randomly and independently drawn out of a {\em finite set}
$\Theta$ with a common prior distribution~$\Gamma$.   Let $\mbf{P}(
\cdot | x, a, f; \theta)$ and $\pi(x, a, f; \theta)$
denote the transition kernel and payoff of a type $\theta$ player.

%The state transition kernel and the
%single period payoff of a player depend on its type. Thus, the state
%transition of player~$i$ with type~$\theta_{i}$ is given as
%\[
%x_{i,t+1} \sim \mbf{P}\left(\cdot \ \Big | \ x_{i,t}, a_{i,t}, \fmi; \theta_{i}\right),
%\]
%and its single period payoff is given as $\pi\big(x_{i,t}, a_{i,t}, \fmi; \theta_{i}\big)%$. Here~$\fmi$ is the population state as defined in equation~\eqref{eqn:actual-dist}.

To analyze a stochastic game with heterogeneous players, we define a
new state as follows. Let  $\xhat = (x, \theta)$ be
an extended state; if a player's extended state is $\xhat$, we interpret it to
mean that the player is in state $x$ and has a type $\theta$.  We let
$\mc{\hat{X}} = \mc{X} \times \Theta$ denote the expanded state
space.  Let $\hat{f}$ denote a population state over the expanded
state space, i.e., $\hat{f}$ is a distribution over $\mc{\hat{X}}$.
Given $\hat{f}$, we define $F(\hat{f}) \in \mfr{F}$ by:
\[ F(\hat{f})(x) = \sum_{\theta} \hat{f}(x, \theta). \]
We have the following two definitions:
\begin{align*}
 \hat{\pi}(\hat{x}, a, \hat{f}) &= \pi(x, a, F(\hat{f}); \theta);\\
\hat{\mbf{P}}(\hat{x}' | \hat{x}, a, \hat{f}) &= \left\{
\begin{array}{ll}
0,&\ \text{if}\ \theta' \neq \theta;\\
\mbf{P}(x' | x, a, F(\hat{f}); \theta),&\ \text{if}\ \theta' = \theta.
\end{array}
\right.
\end{align*}
These definitions simply map the payoff and transition kernel with
respect to the extended state back to the payoff and transition kernel
in the original game.  Now observe that in the new game defined in
this way, it can be verified that if the original game satisfied
Assumptions \ref{as:continuity}, \ref{as:UIC} or \ref{as:convexity}, and~\ref{as:compactness} for each $\theta$, then the extended game
satisfies the same assumptions as well.  Thus all our preceding
results apply even in games with heterogeneous players. Because
strategies are a function of the extended state,  in this case
players of different types will use different strategies.


% Let $\hat{f}_{-i,t}^{(m)}(\hat{y})$ denote the fraction of players (excluding player~$i$) that have their extended state as $\hat{y} = (y, \theta)$ at time~$t$. That is,
% \[
% \hat{f}_{-i,t}^{(m)}(\hat{y}) = \frac{1}{m-1}\sum_{j\neq i} \indic{\{\xhat_{j,t} = \hat{y}\}}.
% \]
% Thus, $\hat{f}_{-i,t}^{(m)}$ is the population state over the extended state space. It is easy to verify that for $\hat{y} = (y, \theta)$, we have
% \[
% \fmi(y) = \sum_{\theta \in \Theta}\hat{f}_{-i,t}^{(m)}(y, \theta).
% \]
% With this extended state space, the state transition of players can be written as
% \[
% \xhat_{i, t+1} \sim \mbf{\hat{P}}\left(\cdot \ \Big | \  \xhat_{i,t}, a_{i,t}, \hat{f}_{-i,t}^{(m)}\right),
% \]
% and the single period payoff of every player is given as~$\hat{\pi}\big(\xhat_{i,t}, a_{i,t}, \hat{f}_{-i,t}^{(m)}\big) = \pi\big(x_{i,t}, a_{i,t}, \fmi; \theta_{i}\big)$. Note that with the extended state space all players have same transition kernel~$\hat{P}$ and same payoff~$\hat{\pi}$. Furthermore, the population state~$\hat{f}_{-i,t}^{(m)}$ is over the extended state space. Thus, the anonymous stochastic game with heterogeneous players can be written as anonymous stochastic game with uniform players.

% \newsa{Add verification of assumptions?}

\subsection{Coupling Through Actions} \label{se:couple actions}

In the main development of this paper, we considered anonymous
stochastic games where players are coupled to each other via the
population state as defined in equation~\eqref{eqn:actual-dist}; note,
in particular, that the population state gives the fraction of players
at each state.  As discussed in the Introduction, however, in many
models of interest the transition kernel and payoff of a player may
depend on both the current state and {\em current actions} of other
players.  In particular, the examples in Sections
\ref{subsec:learning} and \ref{subsec:SC} are models where players are
coupled through their actions.

To formally model such a scenario, we consider an~$m$ player
stochastic game being played in discrete time over the infinite
horizon, where again the payoff and transition kernel of a player are
denoted {by} $\pi(x, a,f)$ and $\mbf{P}(\cdot | x, a, f)$
respectively.\footnote{For the purposes of this subsection we assume
  players are homogeneous.}  However, we now assume that $f$ is a
distribution over both states and actions.  We refer to $f$ as the
{\em population state-action profile} (to distinguish it from just the
population state, which is the marginal distribution of $f$ over
$\mc{X}$).  For simplicity, since the prior development in this paper
assumes state spaces are discrete, for the purposes of this subsection
we restrict attention to a game with a {\em finite} action space $S
\subset \Z^k$, cf. Definition \ref{def:finiteaction}; in particular,
we assume that players maximize payoffs with respect to randomized
strategies over~$S$.  Thus the population state-action profile is a
distribution over $\mc{X} \times S$.

We again let $x_{i,t} \in \mc{X}$ be the state of player~$i$ at
time~$t$, where $\mc{X} \subseteq \Z^{d}$. We let~$s_{i,t} \in S$ be
the (pure) action taken by player~$i$ at time~$t$.  Let $\fmi$ denote
the empirical population state-action profile at time $t$ in an
$m$-player game; in other
words, $f_{i,t}^{(m)}(x,s)$ is the fraction of players other than~$i$
at state $x$ who play $s$ at time $t$.  With these definitions,
$x_{i,t}$ evolves according to the transition kernel $\mbf{P}$ as before, i.e.,
$x_{i,t+1} \sim \mbf{P}(\cdot | x_{i,t}, a_{i,t}, f_{-i,t}^{(m)})$.

A player acts to maximize their expected discounted payoff, as before.
Note that a potential challenge here is that a player's time $t$
payoff and transition kernel depend on the actions of his competitors, which are chosen
{\em simultaneously} with his own action.  Thus to evaluate the time~$t$ expected  payoffs and transition kernel, a player must take an expectation with respect to
the randomized strategies employed by his competitors.

Our first step is to extend the appropriate assumptions to this game
model.  Let $\mfr{F}$ now denote the set of all distributions over $\mc{X}
\times S$, and let $\mfr{F}_p$ denote the set of all distributions in
$\mfr{F}$ with finite $\onep$-norm as before.  Assumptions
\ref{as:continuity} and \ref{as:compactness} thus extend naturally to
games with coupling through actions, with these new interpretations of
$\mfr{F}$ and $\mfr{F}_p$.

The AME property continues to hold for games with coupling through
actions.  Recall that in the proof of Theorem \ref{th:AME}, we
establish that if $(\mu,f)$ is a stationary equilibrium, then
$\|f_{-i,t}^{(m)} - f\|_{\onep} \to 0$ almost surely for all $t$, if
players' initial states are sampled independently from $f$, all
players other than $i$ follow strategy $\mu$, and player $i$ follows
any strategy.  (See Lemma \ref{lem:convergence-of-f} in the Appendix.)
In a game with coupling through actions, $f_{-i,t}^{(m)}$ also tracks
the empirical distribution of players' actions.  However, since all
players other than $i$ use the same oblivious strategy $\mu$, and
since the base action space $S$ is finite, it is straightforward to
extend the argument of Lemma~\ref{lem:convergence-of-f} to the current
setting. The remainder of the existing proof of Theorem~\ref{th:AME}
carries over essentially unchanged under Assumption~\ref{as:continuity}; for brevity we omit the details.

Next, recall that to prove existence of a stationary equilibrium, we consider two maps: $\mc{P}(f)$ (which identifies
the set of optimal oblivious strategies given $f$), and $\mc{D}(\mu,f
)$ (which identifies the set of invariant distributions of the Markov
process induced by $\mu$ and $f$).  The analysis of $\mc{P}(f)$
proceeds exactly as before (but with randomized strategies, as
  discussed in Section \ref{ssec:finiteaction}).  However, in a game
with coupling through 
actions, we redefine $\mc{D}(\mu, f)$ to be the
set of invariant distributions over $\mc{X} \times S$ induced by $\mu$
and $f$.  In other words, $f' \in \mc{D}(\mu, f)$ if and only if there
exists a distribution $g$ over $\mc{X}$ such that the following two conditions hold:
\begin{align*}
g(x') &= \sum_x g(x) \mbf{P}(x' | x, \mu(x),f),\ \text{for all}\ x';\\
f'(x, s)  &= g(x) \cdot \mu(x)(s),\ \text{for all}\ x,s.
\end{align*}
Note that here $\mu(x)(s)$ is the probability assigned to
pure action $s$ by the randomized strategy $\mu$ at state $x$.
The first equation requires that $g$ is an invariant distribution of
the state Markov process induced by $\mu$ and $f$ (recall Definition
\ref{def:finiteaction} of the transition kernel with mixed
actions).  The second 
equation requires $f'$ to be derived from $g$ in the natural way, via $\mu$.
As before, we let $\Phi(f) = \mc{D}(\mc{P}(f), f)$.

It is now straightforward to show that if Assumption~\ref{as:continuity} holds, then the result of Proposition~\ref{prop:uhc} holds, i.e., $\Phi$ has a closed graph.  Further, if Assumptions~\ref{as:continuity} and~\ref{as:compactness} hold, then
the result of Proposition~\ref{prop:compactness} holds as well.  From this and the result in Proposition~\ref{prop:finiteconvex} we conclude that under those assumptions, a stationary equilibrium
exists, and all SE are light-tailed (i.e., have finite $\onep$ norm).  The arguments involved are analogous to the existing proofs,
and we omit the details.


% In other words, consider the following transition kernel on
% the extended state space $\mc{X} \times S$:
% \begin{equation}
% \label{eq:hatP}
%  \hat{\mbf{P}}_{\mu,f}(x', s' | x, s) = \mbf{P}(x' | x, s, f) \cdot
% \mu(x')(s').
% \end{equation}
% (The second term on the right hand side is the probability assigned to
% pure action $s'$ by the randomized strategy $\mu$ at state $x'$.)
% In a stationary equilibrium for a game with coupling through actions,
% we require the population state-action profile to be an invariant
% distribution of a Markov process with transition kernel
% $\hat{mbf{P}}_{\mu,f}$.  Thus we let $\mc{D}(\mu, f)$ be the set of
% invariant distributions of $\hat{\mbf{P}}$.\footnote{Note that we can also
% find such an invariant distribution by first finding an invariant
% distribution of the state Markov process $\mbf{P}(\cdot | x, \mu(x),
% f)$, and then expanding that to a distribution over $\mc{X} \times S$
% via the policy $\mu$.

% To analyze this game, we define an extended state as $\xhat_{i,t} =
% \big(x_{i,t-1}, a_{i,t-1}\big)$. Thus, $\xhat_{i,t}$ consists of the
% state and action of player~$i$ at time~$t-1$.  Thus consider a new
% game with state space $\hat{\mc{X}} = \mc{X} \times S$.  Letting
% $\hat{x} = (x,a)$ and $\hat{x}' = (x',a')$, we have the following two definitions:
% \begin{align*}
%  \hat{\pi}(\hat{x}, \hat{a}, f) &= \frac{1}{\beta}\pi(x, a, f);\\
% \hat{\mbf{P}}(\hat{x}' | \hat{x}, \hat{a}, f) &=
% \left\{
% \begin{array}{ll}
% 0,&\ \text{if}\ a' \neq \hat{a};\\
% \mbf{P}(x' | x, a, f); \theta),&\ \text{if}\ a' = \hat{a}.
% \end{array}
% \right.
% \end{align*}
% In particular, observe that with the definition of the kernel, the
% current extended state is actually the state and action of the {\em last}
% time step.  Further, note that the kernel $\hat{\mbf{P}}$ is multiplicatively
% separable in state and action, since the action component of the next
% extended state is deterministic.

% Let $\hat{f}_{-i,t}^{(m)}(\hat{y})$ denote the fraction of players (excluding player~$i$) that have their extended state as $\hat{y} = (y, a)$ at time~$t$. That is,
% \[
% \hat{f}_{-i,t}^{(m)}(\hat{y}) = \frac{1}{m-1}\sum_{j\neq i} \indic{\{\xhat_{j,t} = \hat{y}\}}.
% \]
% Since the extended state $\xhat_{j,t} = (x_{j,t-1}, a_{j,t-1})$, it
% follows that $\hat{f}_{-i,t} = f_{-i,t-1}$, where the latter is the
% time $t-1$ population state-action profile.  Thus we have $\hat{\pi}(\hat{x}_{i,t}, a_{i,t},
% \hat{f}_{-i,t}^{(m)}) = (1/\beta)\pi(x_{i,t-1}, a_{i,t-1}, f_{-i,t-1}^{(m)})$, so in particular
% expected discounted payoffs are identical in the extended game and the
% original game.  Suppose we extend Assumptions \ref{as:continuity} and
% \ref{as:compactness} by considering $f$ as a population state-action
% profile rather than just a population state, wherever it appears.  It
% is now straightforward to check that if these
% extensions of Assumptions \ref{as:continuity} and/or
% \ref{as:compactness} are satisfied by the original game, then
% they hold, respectively, for the extended game as well.  Thus by
% expanding the state space as described here, all the results of the
% preceding analysis carry through to games where players are coupled
% through actions as well.

We conclude by commenting on the restriction that the action space
must be finite.  From a computational standpoint this is not very
restrictive, since in many applications discretization is required or
can be used efficiently.  From a theoretical standpoint, we can
analyze games with general compact Euclidean action spaces using
techniques similar to this paper, at the expense of additional
measure-theoretic complexity, since now the population state-action
profile is a measure over a continuous extended state space.


% Since the action set~$\mc{A}$ is finite, the extended state~$\xhat_{i,t} \in \mc{X} \times \mc{A} \subset \Z^{d+q}$. We let $\hat{f}_{-i,t}^{(m)}$ be the population state (from player $i$'s point of view) at time~$t$. Note that $\hat{f}_{-i,t}^{(m)}$ is the distribution over state and action space. With this extended state, we can write the state transition as:
% \[
% \xhat_{i,t+1} \sim \mbf{\hat{P}}\left(\cdot \ | \ \xhat_{i,t}, a_{i,t}, \hat{f}_{-i,t}^{(m)}\right)
% \]
% The single period payoff of player~$i$ is given as $\hat{\pi}\big(\xhat_{i,t}, a_{i,t}, \hat{f}_{-i,t}^{(m)}\big) = \pi\big(x_{i, t-1}, a_{i, t-1}, f_{-i,t-1}^{(m)}\big)$.
}


==> preamble.tex <==
\RUNAUTHOR{Adlakha et al.}
\RUNTITLE{Equilibria of Dynamic Games with Many Players :}

\TITLE{Equilibria of Dynamic Games with Many Players:\\
Existence, Approximation, and Market Structure\thanks{The authors are
grateful for helpful conversations with Vineet Abhishek, Lanier Benkard, Peter Glynn,
Andrea Goldsmith, Ben Van Roy, and Assaf Zeevi, and seminar
participants at the INFORMS Annual Meeting and the Behavioral and
Quantitative Game Theory Workshop.  This work was 
supported by DARPA under the ITMANET program, and by the National
Science Foundation.}}

\ARTICLEAUTHORS{%
\AUTHOR{Sachin Adlakha}
\AFF{California Institute of Technology,
  Pasadena, CA, 91125, \EMAIL{adlakha@caltech.edu}} %, \URL{}}
\AUTHOR{Ramesh Johari}
\AFF{Department of Management Science and Engineering, Stanford
  University, Stanford, CA, 94305, \EMAIL{ramesh.johari@stanford.edu}}
\AUTHOR{Gabriel Y. Weintraub}
\AFF{Columbia Business School, New York, NY, 10027,
  \EMAIL{gweintraub@columbia.edu}}
%\AUTHOR{Andrea Goldsmith}
%\AFF{Department of Electrical Engineering, Stanford University,
%  Stanford, CA, 94305, \EMAIL{andrea@wsl.stanford.edu}}
% Enter all authors
} % end of the block

\ABSTRACT{In this paper we study stochastic games with many players; such
games are relevant for a wide range of social, economic, and
engineering applications.  The standard solution concept for such
games is {\em Markov perfect equilibrium} (MPE), but it is well known
that MPE computation becomes intractable as the number of players
increases.  Further, MPE demands a perhaps implausible level of
rationality on the part of players in large games.  In this paper we
instead consider {\em stationary equilibrium} (SE), where players optimize
assuming the empirical distribution of others' states remains constant at
its long run average.We make three main contributions.  First, we provide exogenous
conditions over model primitives to ensure stationary equilibria exist, in a general
model with possibly unbounded state spaces.  Second, we show that the
same conditions that ensure existence of SE also ensure that SE is a
good approximation to MPE in large finite games.  Finally, we
consider a series of applications, including dynamic oligopoly models,
supply chain competition, and consumer learning.  These examples
highlight that our conditions amount to a dichotomy between
``decreasing'' and ``increasing'' returns to larger states; SE approximates
MPE well in the former case in which the equilibrium market structure
becomes fragmented in the limit. In the
latter case, SE may not approximate MPE well.} 

